Jellyfish: A Large Language Model for Data Preprocessing

This paper explores the utilization of LLMs for data preprocessing (DP), a crucial step in the data mining pipeline that transforms raw data into a clean format conducive to easy processing. Whereas the use of LLMs has sparked interest in devising universal solutions to DP, recent initiatives in this domain typically rely on GPT APIs, raising inevitable data breach concerns. Unlike these approaches, we consider instruction-tuning local LLMs (7 -- 13B models) as universal DP task solvers that operate on a local, single, and low-priced GPU, ensuring data security and enabling further customization. We select a collection of datasets across four representative DP tasks and construct instruction tuning data using data configuration, knowledge injection, and reasoning data distillation techniques tailored to DP. By tuning Mistral-7B, Llama 3-8B, and OpenOrca-Platypus2-13B, our models, namely, Jellyfish-7B/8B/13B, deliver competitiveness compared to GPT-3.5/4 models and strong generalizability to unseen tasks while barely compromising the base models' abilities in NLP tasks. Meanwhile, Jellyfish offers enhanced reasoning capabilities compared to GPT-3.5. Our models are available at: https://huggingface.co/NECOUDBFM/Jellyfish . Our instruction dataset is available at: https://huggingface.co/datasets/NECOUDBFM/Jellyfish-Instruct .

==> ethics.tex <==
\section*{Ethical Statement}
In this work, we study tuning LLMs for DP. To the best of our knowledge, there is no negative societal impact in this research. 

Despite generative AI used to polish the writing of the paper, we are responsible for all the materials presented in this work.

==> limitations.tex <==
\section*{Limitations}
We investigated six DP tasks in this paper, whereas there are still many other tasks (e.g., data repairing, data fusion, and data transformation). We will investigate them in our future work. 

We discovered that our reasoning data compromises the 13B model's DP performance, possibly because OpenOrca-Platypus2-13B's reasoning and logic do not align well with the underlying logic of DP. In contrast, the 7B and 8B models, derived from native models Mistral-7B and Llama 3-8B, respectively, can benefit from the use of reasoning data. Due to the lack of (approximately) 13B size for these two base models, we cannot deliver better DP performance than the 13B model while preserving the interpretation ability. Nonetheless, we believe that our instruction data can apply to more advanced base models, with which better DP performance and interpretation ability could be both achieved. 

Our prompt is designed as instance-based, rather than the table-based setting which was adopted in many non-LLM approaches. This is partially due to the token limitation of the LLMs we used (e.g., 4096 tokens for a 13B model), and compromises efficiency when we use our models for large-scale datasets. We can use prefix caching to alleviate this issue, as shown in our experiments. 

Another limitation is that LLMs might further introduce errors. For example, there is a chance that the model treats correct values as errors in ED. If we use DI on the entries incorrectly detected, it is possible that errors might be further introduced. Nonetheless, Jellyfish models still report higher accuracy than non-LLM solutions. Furthermore, in the instruction-tuning of Jellyfish, we chose base models that generate content in a safe and responsible way, and tried our best to configure the tuning data to avoid bias or safety issues. 

Furthermore, when using our models for practical data mining pipelines, we also need to carefully consider the issues of preprocessing and postprocessing. For example, the input data may be scanned copies and contain hierarchical tables, while we focus on relational tables in this work.  



==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> vldbinfo.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{XX.XX/XXX.XX}
\newcommand\vldbpages{XXX-XXX}
% issue-specific
\newcommand\vldbvolume{14}
\newcommand\vldbissue{1}
\newcommand\vldbyear{2020}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{https://huggingface.co/NECOUDBFM/Jellyfish}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{plain} 
